Time evolution as an optimization problem: The hydrogen atom in strong laser fields in a basis of time-dependent Gaussian wave packets

Recent advances in attosecond science have made it increasingly important to develop stable, reliable and accurate algorithms and methods to model the time evolution of atoms and molecules in intense laser fields. A key process in attosecond science is high-harmonic generation, which is challenging to model with fixed Gaussian basis sets, as it produces high-energy electrons, with a resulting rapidly varying and highly oscillatory wave function that extends over dozens of {\aa}ngstr\"om. Recently, Rothe's method, where time evolution is rephrased as an optimization problem, has been applied to the one-dimensional Schr\"odinger equation. Here, we apply Rothe's method to the hydrogen wave function and demonstrate that complex-valued Gaussian wave packets with time-dependent width, center, and momentum parameters are able to reproduce spectra obtained from essentially exact grid calculations for high-harmonic generation with only 50-181 Gaussians for field strengths up to $5\times 10^{14}$W/cm$^2$. This paves the way for the inclusion of continuum contributions into real-time, time-dependent electronic-structure theory with Gaussian basis sets for strong fields, and eventually accurate simulations of the time evolution of molecules without the Born-Oppenheimer approximation.

==> alt_intro.tex <==
With advances in attosecond physics in recent decades,~\cite{Corkum2007,Krausz2009,Lewenstein_QO_QI} such as the discovery of high-harmonic generation in gases,~\cite{HHG_discovery_1,HHG_discovery_2} real-time observation of ultra-fast electron dynamics,~\cite{Fohlisch2005} attosecond imaging,~\cite{Haessler2010} and the control of ionization dynamics in noble gases,~\cite{Hutten2018} culminating in the Nobel Prize in Physics in 2023 being awarded to Agostini, Krausz, and L'Huillier,~\cite{NobelPrize} it has become increasingly important to understand, interpret, and predict matter-field interactions on a theoretical level by solving the time-dependent Schrödinger equation (TDSE). Many methods have been developed to solve the TDSE approximately, and they have been applied successfully to atoms and molecules. Methods to accurately solve the TDSE for the interaction between light and atoms using the single-active electron approximation (SAE)\cite{SAE_1,SAE_3} include spatial grid methods,~\cite{Bandrauk} the use of B-splines,~\cite{Bspline_2} time-dependent configuration interaction (TDCI) using large, tailored Gaussian basis sets,~\cite{Luppi,Coccia,Wozniak} and hybrid B-spline/Gaussian basis sets.~\cite{Bspline_1} Time-dependent methods to solve the TDSE for larger electronic systems include time-dependent density functional theory (TDDFT)~\cite{TDDFT} and wave function methods~\cite{Time_dependent_methods,Time_dependent_methods_2,Time_dependent_methods_3,HHG_methods_review} such as multiconfigurational time-dependent Hartree-Fock (MCTDHF) theory,~\cite{MCTDHF1,MCTDHF2} time-dependent coupled-cluster (TDCC) theory,~\cite{TDCC_review} TDCI methods,~\cite{TDCI}, grid and B-spline methods,~\cite{Bspline_3} and hybrid methods.~\cite{Gauss_DVR,Gauss_Bspline}

In addition, methods have been developed to solve the TDSE in a basis of time-dependent Gaussians, where both linear and nonlinear parameters are updated using time-dependent variation principles.~\cite{lubich2005variational} The variational multiconfigurational Gaussian (vMCG) approach, in particular, solves the TDSE using time-dependent Gaussians for the dynamics of molecular nuclei.~\cite{G-MCTDH,vMCG} However, severe numerical instabilities are frequently encountered when time-dependent variation principles are applied to the nonlinear Gaussian parameters,~\cite{Sawada,G-MCTDH,vMCG,KAY1989165,Lee2018,HaakonPhD} leading to unreliable results. While there exist approaches to overcome these issues, they rely on assumptions about the potential and particle locality such as the local harmonic approximation,~\cite{Heller_1975} or they introduce approximations such as frozen Gaussians or independent propagation of Gaussians.~\cite{Heller_1981} Another drawback is that there is no natural way to enlarge the variational space, as there is no obvious way to remove or add Gaussian functions.

For electron dynamics in strong fields, propagating Gaussians in time using a time-dependent variation principle becomes particularly challenging, as the Coulomb potential is not locally harmonic and electrons are inherently delocalized. Gaussians cannot be propagated independently of one another, and electrons can spread over dozens of Ångstrøm. High-harmonic generation (HHG), in particular, is a time-dependent phenomenon that is particularly challenging to model. Qualitatively, HHG can be qualitatively understood in terms of the semi-classical three-step model.~\cite{three_step_model} A driving laser field, typically in the near-infrared spectral region, induces tunnel ionization of an electron (step 1), which is then accelerated away from the nucleus until the direction of the electric field changes (step 2), driving the electron back towards the nucleus, where they recombine with excess energy emitted as ultra-short (trains of) pulses of radiation in the extreme ultraviolet and soft x-ray spectral ranges (step 3). The Lewenstein model\cite{Lewenstein_model} is founded on the three-step model and gives a semi-quantitative account of HHG by describing it fully quantum-mechanically. It relies on several approximations, however. After interaction with the driving laser, the resulting wave function describing the atom or molecule is highly oscillatory and strongly delocalized with significant contributions from the electronic continuum. In order to describe the system accurately, it is hence necessary that a numerical model can incorporate this behavior. In grid calculations, a very large simulation box extending over several hundred Bohr must be used. Approaches using a fixed basis set with time-dependent linear coefficients require a good representation of Rydberg states and the electronic continuum, which can be approximated with basis sets such as Kaufmann functions.~\cite{Kaufmann} Although grid methods give excellent results, they have an unfavorable scaling with the number of electrons $N$, in principle requiring a simulation box of dimension $N^3$, even though this number can be reduced through symmetry considerations and suitable approximations. Both grids and Gaussian basis sets can become very large, and it may additionally be necessary to use a masking function,~\cite{Masking_functions} heuristic lifetime models,~\cite{Klinkusch,Coccia,Coccia2} or complex absorbing potentials~\cite{Manolopoulos,Giovannini,Yu_2018} to suppress nonphysical reflections from the boundaries of the simulation box (finite Gaussian basis sets implicitly define a simulation box, too). Depending on the size of the grid or the basis set, this procedure can be necessary to obtain qualitatively correct HHG spectra even for low intensities of the driving laser, and unless one uses extremely large basis sets or grids, it is crucial for high intensities.

In this work, we use Rothe's method,~\cite{Rothe1930_MA} which \citeauthor{kvaal2023need}~\cite{kvaal2023need} recently applied to study a one-dimensional hydrogen-like atom interacting with a strong laser field. \textcolor{green!70!black}{Previous applications of Rothe's method in quantum mechanics include the propagation of neural-network quantum states~\cite{Gutierrez2022} and solving the quantum-classical Liouville equation.~\cite{Horenko2004adaptive}} \citeauthor{kvaal2023need} used an adaptive basis of complex-valued Gaussians
to express the electronic wave function and determined both the basis-set dimension and the linear and nonlinear parameters associated with each Gaussian basis function at every time step of the simulation. While Rothe's method is completely general and does not require underlying assumptions about the way the wave function is represented at each time step, a time-dependent Gaussian basis can provide a very compact representation of the wave-function evolution during interaction with strong laser fields.~\cite{Wozniak_Gaussians} 

%The HHG process is a process where using a time dependent variational  principle with Gaussians is difficult due to the complexity of the resulting wave function compared to the initial wave function, the delocalization of only small parts of the wave function, the Coulomb potential, and the oscillatory behaviour of the wave function leading to an inter-depencence of Gaussians. However, using Rothe's method, where time-evolution is rephrased as an optimization problem, many of the inherent problems using a TDVP with Gaussians, are alleviated. \par 

The structure of this paper is as follows. In Sec.~\ref{sec:Methods}, we first describe Rothe's method in detail and how it reformulates time evolution as an optimization problem. This is followed by a description of the basis set and the Hamiltonian we are using. We describe how the error in Rothe's method relates to the variance of a wave function for a given Hamiltonian. We then describe how the optimization is carried out, with particular focus on adding and removing Gaussian basis functions. In Sec.~\ref{sec:Results}, we present HHG spectra produced using Rothe's method and compare them to HHG spectra obtained using DVR and Kaufmann basis functions with a heuristic lifetime model. We conclude in Sec.~\ref{sec:Conclusion} with a discussion of the strengths and shortcomings of Rothe's method, and how Rothe's method might be used for modelling larger systems.

